SE(3) Equivariant Graph Neural Networks with Complete Local Frames

Group equivariance (e.g. SE(3) equivariance) is a critical physical symmetry in science, from classical and quantum physics to computational biology. It enables robust and accurate prediction under arbitrary reference transformations. In light of this, great efforts have been put on encoding this symmetry into deep neural networks, which has been shown to improve the generalization performance and data efficiency for downstream tasks. Constructing an equivariant neural network generally brings high computational costs to ensure expressiveness. Therefore, how to better trade-off the expressiveness and computational efficiency plays a core role in the design of the equivariant deep learning models. In this paper, we propose a framework to construct SE(3) equivariant graph neural networks that can approximate the geometric quantities efficiently. Inspired by differential geometry and physics, we introduce equivariant local complete frames to graph neural networks, such that tensor information at given orders can be projected onto the frames. The local frame is constructed to form an orthonormal basis that avoids direction degeneration and ensure completeness. Since the frames are built only by cross product operations, our method is computationally efficient. We evaluate our method on two tasks: Newton mechanics modeling and equilibrium molecule conformation generation. Extensive experimental results demonstrate that our model achieves the best or competitive performance in two types of datasets.

==> background.tex <==
\section{Preliminary}
%we first introduce some basic concepts on the notion of equivariance and tensor field and then describe the scalarization technique from differential geometry. Finally, we define the `vector field' as the differential of a many-body system.  
In this section, we set up the necessary mathematical preliminaries for understanding the follow-up sections.
Let $\mX=(\vx_1,\dots,\vx_N) \in \mathbb{R}^{N\times 3}$ be a many-body system (3D point clouds) living in $\mathbb{R}^3$, where $N$ is the number of particles. If the system is dynamical, then we use $\vx_i(t)$ to denote the position of the particle $i$ at time $t$. Given a particle $\vx_i(t)$, define neighbor $\mathcal{N}(\vx_i(t))$ as the particles that react with $\vx_i(t)$. Let $\times$ denote the cross product of two vectors, and $\otimes$ denote the tensor product operation.   
\paragraph{SE(3) group and Equivariance}
%Throughout the article, $\cdot\ $\  denotes the inner product of two vectors, $\times\ $\  means the cross product of two vectors, and $\otimes\ $\  denotes the tensor product of two tensors. 
%Consider  
In Euclidean space $\mathbb{R}^3$, %equipped with the standard Euclidean metric
%$g_{ij} = \delta_{ij}$, 
 we consider affine transformations that preserve the distance between any two points, i.e., the isometric group SE(3). We call it the symmetry group w.r.t. the Euclidean metric, and it turns out that SE(3) can be generated by the translation group and the rotation group SO(3) (check appendix \ref{so3} for a definition). 

Once we have a symmetry group, it's valid to define quantities that are ``equivariant'' under the symmetry group. 
Given a function $f: \mathbb{R}^m \rightarrow \mathbb{R}^n$, assuming the symmetry group $G$ acts on $\mathbb{R}^m$ and $\mathbb{R}^n$ and we denote the actions by $T_g$ and $S_g$ correspondingly, then $f$ is $G$-\textbf{equivariant} if
$$f(T_g x) = S_g f(x),\ \ \ \forall x \in \mathbb{R}^m\ \text{and}\ g \in G.$$
For SO(3) group, if \textcolor{red}{$n=1$, i.e., the output of $f$ is a scalar, then the group action on $\mathbb{R}^1$ is the identity map, in this case $f$ should be $SO(3)$-invariant \citep{thomas2018tensor}: $f(gx) = f(x).$}  %the group action on $\mathbb{R}^n$ is the identity map, then $f$ should be $G$-invariant:

The notion of \textbf{tensor field} can be defined for general Riemannian manifold (see Definition 2.1.10 of \citep{jost2008riemannian}). \textcolor{red}{Let {\small$\{\frac{\partial}{\partial x_{i}}\}_{i=1}^3$} and {\small$\{dx^i\}_{i=1}^3$} be the tangent vectors and dual vectors in $\mathbb{R}^3$ respectively}. Then recall the definition of tensor field on $\mathbb{R}^3$ w.r.t. the SO(3) group:
\begin{definition} \label{ten}
A \textbf{(r,\,s)- tensor field} $\theta$ is a multi-linear map from a collection of r dual vectors and s vectors in $\mathbb{R}^3$ to $\mathbb{R}$:
{\small$\theta(x) = \theta^{i_1 \cdots i_r}_{j_1 \cdots j_s}\  \frac{\partial}{\partial x_{i_1}}\otimes \cdots \otimes \frac{\partial}{\partial x_{i_r}}\otimes dx^{j_1} \otimes \cdots \otimes dx^{j_s}.$}
It implies that under SO(3) coordinate transformation $g :=\{g_{ij}\}_{1 \leq i,j \leq 3}$,  the tensor field $\theta$ transforms \textbf{equivariantly}:
{\small$\theta^{i_1' \cdots i_r'}_{j_1' \cdots j_s'} = g_{i_1'i_1}\cdots g_{i_r'i_r}g^T_{j_1j_1'}\cdots g^T_{j_sj_s'} \theta^{i_1 \cdots i_r}_{j_1 \cdots j_s},$}
where $g^T$ is the inverse of $g$.
\end{definition}
\textcolor{red}{The notion of tensor field is introduced for expressing and embedding of geometric and physical quantities, under which the representation satisfies the group \textbf{equivariance}. Therefore, the tensor product is a natural operation to combine two equivariant representations, which can generates another equivariant representation.}%e.g. velocity, momentum, force are order 1 tensors, and the stress–energy tensor is order 2 tensors. As it was shown in section 4 of \citep{dym2020universality}, tensor product of equivariant vectors can be seen a higher-order \textbf{equivariant embedding} of vectors.}

To model a differentiable dynamical system $\mX(t)$, a natural way is to estimate its differential $\frac{d \mX(t)} {d t}$ and apply an ODE solver to integrate the differential to obtain the dynamic trajectory or a state at a given time. Due to the SO(3) symmetry, such differential is a (1,0)-type tensor field, we name it as an \textbf{equivariant vector field}. further illustrations can be found in the appendix \ref{evo}.
\paragraph{Graph neural network}Since many body system modeling is independent of the labeling on the observed particles (permutation equivariance), we will use graph-based message passing mechanism \citep{gilmer2020message} heavily in this paper. Given a graph$G = (V(G),E(G))$ with nodes $v_i \in V(G)$ and edges $e_{ij} \in E(G)$, let $h_i$ and $t_{ij}$ be the feature vectors aatached to each node and edge. Then recall how EGNN \citep{satorras2021en} compute message $m_ij$ from node $i$,$j$:
\begin{align}
\label{eq:egnnmessages}
m_{ij} &= \text{MLP}(\mathbf{h}_i, \mathbf{h}_j, \lVert \vx_j - \vx_i \rVert^2)\\
&= \sigma(W^{(k)} (\ldots(\sigma(W^{(1)} (\mathbf{h}_i, \mathbf{h}_j, \lVert \vx_j - \vx_i \rVert^2))) \ ,    
\end{align}
with non-linear activation $\sigma$. %Then the node feature is updated by
%$$\mathbf{h}_i^{l+1} = \phi_n (\mathbf{h}_i^{l},\sum_{j \in \mathcal{N}(i)} m_{ij}).$$
%The vector output is updated by
%$$\vx_i^{l+1} = \vx_i^l + C \sum_{j \neq i} (\vx_j^l - \vx_i^l) \phi_x (m_{ij}).$$


 %Most 3D real-world scenarios adopt \textbf{first-order} and \textbf{second-order} equivariant vector fields to depict their dynamic evolving mechanisms, which are also the modeling targets in this paper. Graident fields are first order equivariant vector fields, further illustration can be found at appendix. A typical second-order vector field is the acceleration field of Newtonian systems. 



==> property.tex <==
\subsubsection{Molecular Property Prediction}
\label{app:property}
Chemical property prediction is another standard task defined on the QM9 dataset. These properties are invariant to arbitrary translation and rotation transformations, which provides a natural platform to validate our ClofNet. 

\paragraph{Implementation Details. } We follow the data partitions reported in \citep{anderson2019cormorant, satorras2021en}, $100K$ molecules for training, $18K$ for validation and $13K$ for testing. We estimate all of 12 chemical properties for each molecule by optimizing the Mean Absolute Error (MAE) between predictions and labels. For model implementations, we adopt EGNN as our codebase\footnote{\url{https://github.com/vgsatorras/egnn}}, however, extra imposing our scalarization block on the original framework, trying to demonstrate the expressiveness of our method for complex geometric information. In detail, the model receives the atomic positions and the atom properties as input. Following EGNN, our ClofNet also consists of 7 layers, 128 hidden dimensions per layer and the Swish activation function as a non-linearity. We include Schent \citep{schutt2017schnet}, Cormorant \citep{anderson2019cormorant}, L1Net \citep{miller2020relevance}, LieConv \citep{finzi2020generalizing}, %DimeNet++ \citep{klicpera2020directional}, 
TFN \cite{thomas2018tensor} and SE(3)-Tr. \citep{fuchs2020se} %SphereNet \citep{liu2021spherical} and PairNN \citep{schutt2021equivariant} 
as our baselines. 
% These baselines 

\paragraph{Results. }As shown in Table \ref{table:qm9_proper_com}, ClofNet outperforms its architecture counterpart, EGNN\citep{satorras2021en} on all properties, demonstrating its more powerful capacity on handling geometric information. Moreover, we find that ClofNet achieves a competitive performance on most non-energy variables, however, exhibits a poorer performance on the energy variables ($G$, $H$, $U$, $U_0$). These results imply that it is necessary to incorporate other target-specific inductive bias into models for those energy variables. 
For example, SphereNet adopt complex spherical harmonics and spherical Bessel functions as their feature embedding functions, which mimics the physical solution of the Schrödinger equation. In contrast, ClofNet doesn't include any complex feature engineering operations, making it more simple and time-efficient. We will leave the study that how to effectively combine ClofNet with other chemical or physical priors as our future work.  

\begin{table*}[t]
  \caption{MAE for molecular property prediction on QM9 dataset. 
   * denotes the method uses different train/val/test partitions from other methods.
  }
  \label{table:qm9_proper_com}
  \centering
  \begin{tabular}{ccccccccccccc}
    \toprule
      Task & $\alpha$ & $\Delta\epsilon$ & $\epsilon_{\text{HOMO}}$ & $\epsilon_{\text{LUMO}}$ & $\mu$ & $C_v$ & $G$ & $H$ & $R^2$ & $U$ & $U_0$ & zpve\\
      Units & bohr$^3$ & meV & meV & meV & %D & cal/mol K & meV & meV & bohr$^3$ %& meV & meV & meV\\
    \midrule
     GNN & 0.01309 & 0.01371	& 0.03055 & \\
    NMP & .092 & 69 & 43 & 38 & .030 & .040 & 19 & 17 & .180 & 20 & 20 & 1.50 \\
    SchNet* & .235 & 63 & 41 & 34 & .033 & .033 & 14 & 14 & .073 & 19 & 14 & 1.70 \\
    Cormorant & .085 & 61 & 34 & 38 & .038 & .026 & 20 & 21 & .961 & 21 & 22 & 2.02 \\
    L1Net & .088 & 68 & 46 & 35 & .043 & .031 &14 & 14 & .354 & 14 & 13 & 1.56\\
    LieConv & .084 & 49 & 30 & 25 & .032 & .038 & 22 & 24 & .800 & 19 & 19 & 2.28\\
    TFN & .223 & 58 & 40 & 38 & .064 & .101 & - & - & - & - & - & -\\
    SE(3)-Tr. & .142 & 53 & 35 & 33 & .051 & .054 & - & - & - & - & - & - \\
    DimeNet++* & \textbf{.043} & \textbf{32} & 24 & 19 & .029 & .023 & \textbf{7} & \textbf{6} & .331 & 6 & 6 & 1.21 \\
    SphereNet* & .046 & \textbf{32} & \textbf{23} & \textbf{18} & .026 & \textbf{.021} & 8 & \textbf{6} & .292 & 7 & 6 & 1.12 \\
    PaiNN* & .045 & 45 & 27 & 20 & \textbf{.012} & .024 & \textbf{7} & \textbf{6} & \textbf{.066} & \textbf{5} & \textbf{5} & 1.28 \\
    EGNN & .071 & 48 & 29 & 25 & .029 & .031 & 12 & 12 & .106 & 12 & 12 & 1.55 \\ \midrule
    ClofNet & .069 & 44 & 27 & 22 & .027 & .028 & 11 & 11 & .123 & 11 & 11 & 1.53\\
    \bottomrule
  \end{tabular}
  \vskip -0.2in
\end{table*}

==> related_work.tex <==
\section{Related Work}
\textbf{Equivariant neural network. }
Various symmetries are considered to be embedded into the network for different tasks. 
Vanilla CNN models are naturally translation invariant, and more works on 2D-symmetry include \citep{he2021efficient,franzen2021general,dieleman2016exploiting,cohen2016group,cohen2016steerable,weiler2019general,shen2020pdo}.
Another common symmetry for 3D objects is SO(3) group \citep{esteves2019equivariant,esteves2019cross,worrall2018cubenet,kondor2021fully}. 
In terms of methodology, existing equivariant networks 
can be roughly classified into two categories by whether conducting all operations in the original space or not.
The first category of methods lift the data into high-dimensional spaces (e.g., lie group) or introduce equivariant functions (e.g., spherical harmonics) to preserve equivariance \citep{worrall2017harmonic, thomas2018tensor, kondor2018clebsch, weiler2018learning, weiler20183d, weiler2019general, esteves2020spin,romero2020attentive,klicpera2020directional, anderson2019cormorant,batzner2021se}. They exhibit sufficient expressive power but usually bring extra computational costs for calculating spherical harmonic embedding (steerable features \citep{2110.02905}) or performing integration on Lie groups. 

Our work follows methods of the second category that operates on the original space in a computationally efficient way \citep{schutt2018schnet,kohler2019equivariant,shi2021learning,deng2021vector}. However, most of these approaches (e.g., EGNN \citep{satorras2021en}) abandon a certain amount of geometric (tensor) information, causing their expressive power to be restricted (on the other hand, the expressive power of TFN equivariant network \citep{thomas2018tensor} does have theoretical guarantees \citep{dym2020universality}). Recall EGNN algorithm (\ref{eq:egnnmessages}), although the messages are fully non-linear, only the invariant distance feature $\lVert \vx_j - \vx_i \rVert$ is fed into the model. On the other hand, the success of \citep{ 2110.02905,batzner2021se} have demonstrated the effectiveness for integrating sophisticated geometric and physical features in a non-linear way by equivariant function embedding (and second hop scalar features \citep{klicpera2020directional}). Although implementing geometric features by spherical harmonics and CG tensor product are manifestly equivariant, this is not the only way. Although \citet{he2021efficient} only deals with 2D-symmetry, theorem 1 of \citet{he2021efficient} gave a criterion holds on judging whether a message aggregation operation is equivariant for a general group. All the above models are sub-solutions of this criterion.%In fact, there exists a criterion on judging whether a message aggregation operation is equivariant from theorem 1 of \citep{he2021efficient} :
%$$\mathbf{f}^{l+1} (g) = \sum_{\Tilde{g} \in G} m_{g,\Tilde{g}} (\mathbf{f}^{l}(g),\mathbf{f}^{l}(\Tilde{g}))$$
%is equivariant w.r.t group $G$ iff
%\begin{equation} \label{efficient}
%\sum_{\Tilde{g} \in G} m_{g,\Tilde{g}} = \sum_{\Tilde{g}} \Tilde{m}_{g^{-1}\Tilde{g}} (\mathbf{f}^{l}(g),\mathbf{f}^{l}(\Tilde{g})) \end{equation}
%for some function $\Tilde{m}_{\Bar{g}}$, which is indexed by a single group element $\Bar{g} \in G$. Although \citet{he2021efficient} only deals with 2D-symmetry, this criterion holds for a general group. Since we can always
%use a lifting operation to lift the original $\mathbb{R}^n$ to the feature maps on $G$, the criterion is general. One merit of this formalization is that higher-order steerable feature vectors can be implemented as higher-order embeddings of the input vectors with the only restriction that (\ref{efficient}) hold. It's also easy to check that steerable convolutions are special cases that satisfy (\ref{efficient}). 

Different from the existing methods, we propose a flexible and efficient architecture that avoids complex vector-level transformations while preserving complete geometric information through the equivariant basis \textcolor{red}{(see the discussion at the end of section 3 and appendix \ref{inc})}. As we have discussed in the methodology section, fixing an equivariant basis is equivalent to fixing a coordinate frame, and any two frames are connected by a $g\in G$. Moreover, \citet{2110.02905} argued the importance of injecting steerable features. %From the definition of tensor fields and the tensor product equivariant bases defined by (\ref{tensor product bases}), we already find a clue on how do higher order equivariant embeddings of the input's vector. 
Recall the two essential ingredients of encoding steerable \citep{freeman1991design} geometric and physical features (see (6) of \citep{2110.02905}) are spherical harmonic embeddings and CG tensor product. More precisely, we take a spherical embedding of an input vector as a steerable feature, and update the node features (tensor type) by taking CG tensor product with the current node features. However, the message from section 4 of \citep{dym2020universality} indicates that the computational expensive SO(3) representations (spherical harmonics and CG decomposition) bring can be realized by direct tensor product (formula (\ref{tensor product bases}) is a special case of generating tensor product equivariant bases from our equivariant basis). Now it's necessary to show how EVFN performs direct tensor product under scalarization. We take a simple example of the inner product between two order one vectors: $\mathbf{\theta}_1 = \theta_1^a \va + \theta_1^b \vb + \theta_1^c \vc$ and  $\mathbf{\theta}_2 = \theta2^a \va + \theta_2^b \vb + \theta_2^c \vc$, under equivariant basis $(\va,\vb,\vc)$. Then the tensor product gives:
\begin{align} \nonumber
 \mathbf{\theta}_1 \otimes \mathbf{\theta}_2 =&  \theta_1^a  \cdot \theta_2^a \va \otimes \va +  \theta_1^b  \cdot \theta_2^b \vb \otimes \vb + \theta_1^c  \cdot \theta_2^c \vc \otimes \vc\\\nonumber
 &+ \theta_1^a  \cdot \theta_2^b \va \otimes \vb + \theta_1^b  \cdot \theta_2^a \vb \otimes \va\\ \nonumber
& + \theta_1^a  \cdot \theta_2^c \va \otimes \vc + \theta_1^c  \cdot \theta_2^a \vc \otimes \va\\ \label{product}
 &+ \theta_1^b  \cdot \theta_2^c \vb \otimes \vc + \theta_1^c  \cdot \theta_2^b \vc \otimes \vb.
\end{align}
Under scalarization, the output of this tensor product is represented by the set containing second order polynomials of the invariant scalars ($\{\theta_1^a \dots \theta_2^c\}$) defined by (\ref{scalar}).
%therefore, although we prove the equivariance of our model in another way, it's not hard to check (\ref{efficient}) directly.     
 

%\textcolor{red}{ Essentially, the scalarization is also adopted by EGNN, which is only computed from one basis and EVFN extends the one basis (i.e., radical direction $\vx_i - \vx_j$) in EGNN into a tuple of bases for information lossless. }


